Empirical Study of the Docker Smells Impact on the Image Size

Docker, a widely adopted tool for packaging and deploying applications leverages Dockerfiles to build images. However, creating an optimal Dockerfile can be challenging, often leading to "Docker smells" or deviations from best practices. This paper presents a study of the impact of 14 Docker smells on the size of Docker images. To assess the size impact of Docker smells, we identified and repaired 16 145 Docker smells from 11 313 open-source Dockerfiles. We observe that the smells result in an average increase of 48.06 MB (4.6%) per smelly image. Depending on the smell type, the size increase can be up to 10%, and for some specific cases, the smells can represent 89% of the image size. Interestingly, the most impactful smells are related to package managers which are commonly encountered and are relatively easy to fix. To collect the perspective of the developers regarding the size impact of the Docker smells, we submitted 34 pull requests that repair the smells and we reported their impact on the Docker image to the developers. 26/34 (76.5%) of the pull requests have been merged and they contribute to a saving of 3.46 GB (16.4%). The developer's comments demonstrate a positive interest in addressing those Docker smells even when the pull requests have been rejected

==> dataset_comparison.tex <==

% \input{figures/violations_distribution_binnacle} 
\input{figures/violations_distribution.tex}

Finally, we compare the results on Binnacle Dataset with the new dataset.
\autoref{fig:distribution_smell_binnacle_dataset} presents the distributions of the number of smells per Dockerfile in Binnacle and the new dataset respectively.
The two figures are relatively similar however \tool Dataset seems to have slightly more Dockerfiles with two and three smells while the Binnacle dataset has more Dockerfiles with one smell.
While the number of Dockerfiles without smell slightly increased as observed by previous studies \cite{lin2020large,EngH21}.
The increase in the number of smells per Dockerfile is probably due to the fact that the number of instructions per Dockerfile has increased by $1/3$ between the two years from an average of \np{12.45} to \np{18.4} (median \np{9} and \np{12}) respectively. 

==> dinghy.tex <==
\subsection{\astTool}\label{sec:asttool}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\columnwidth]{figures/DockerNode.pdf}
%     \caption{DockerNode class diagram}
%     \label{fig:DockerNodeAst}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/pretty-print.png}
    \caption{\astTool pretty print feature.}
    \label{fig:pretty-print}
\end{figure}

\astTool is a library to parse, query, manipulate and reprint Dockerfiles written in \np[k]{3.68} lines of TypeScript. 
It has been designed to make it easy to refactor Dockerfiles by lowering the entry costs of analyzing and transforming Dockerfiles.
\astTool is written in TypeScript to be compatible with Visual Studio Code, one of the most popular IDE\footnote{\url{https://pypl.github.io/IDE.html} visited on \today} and with the browser to increase its adoption and all tools that will depend on it, such as \tool and its web demo \url{\urlDemo}.

\astTool relies on two existing libraries to parse Docker instructions and Bash script: \href{https://www.npmjs.com/package/dockerfile-ast}{dockerfile-ast} and \href{https://www.npmjs.com/package/mvdan-sh}{mvdan-sh}.
The two ASTs are then combined into a unified and consistent AST that can be used to manipulate Docker and Bash nodes transparently. 
In total, we define \np{141} node types, \np{100} bash nodes, \np{41} Docker nodes.
% All nodes in \astTool inherit from DockerNode (see \autoref{fig:DockerNodeAst}) which provides most of the features to manipulate and navigate the Dockerfile AST.
%The string representation of the bash script had to be pre-processed before providing it to mvdan-sh.
\astTool and its documentation are available on GitHub \cite{tool}.

\astTool has a strong focus on refactoring which means that the AST should be easily manipulated but also that the code transformation does not break the code formatting of the Dockerfile.
\astTool is able to reprint the Dockerfile AST with minimal changes compared to the original formatting.
We call this feature pretty print. This feature is illustrated in \autoref{fig:pretty-print}.
We handle this complex problem by only reprinting the nodes that were modified and otherwise reusing the content that was written by the developers.
To be able to do so, we need to track accurately the modifications that have been done on the AST and have accurate positions of each node to be able to find the textual representation of the node in the original Dockerfile. 
Unfortunately, the positions were not always accurate which reflected poor performance of the pretty print before fixing the positions.
We also had to unify the position between the Dockerfile AST and the Shell AST since they were parsed separately.
Additionally, all white spaces (indentations, new lines, and spaces) of the Dockerfiles are reprinted following common practices which produce reliable results according to our tests.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/query.png}
    \caption{Query features of \astTool.}
    \label{fig:query}
\end{figure}

Being able to navigate the AST is one of the most important features of an AST library. 
\astTool supports the traditional navigation features such as getting the parent and the children but it also supports, as presented in \autoref{fig:query}, a query system.
The query allows finding nodes that match a specific pattern.
The query system uses the node types but also annotations and node values.
In \astTool, it is indeed possible to annotate each node which is particularly useful when a multiple steps analysis is required. 
The results from the previous analysis can be used in the following ones.
This allows for doing complex searches with relatively simple queries.
This will be extensively used by \tool.


==> figures/violations_distribution.tex <==
\begin{figure}[t]
  \centering
  \begin{tikzpicture}
    \begin{axis}[
        ybar,
        xmin = -0.5,
        xmax = 7.5,
        ymin = 0,
        %       ymax = 35,
        bar width = 6.5mm,
        axis x line* = bottom,
        axis y line* = left,
        % y axis line style= { draw opacity=0 },
        % ytick=\empty,
        ylabel= \# Dockerfiles,
        width= 0.48\textwidth,
        height = 0.22\textwidth,
        point meta={y*100/\nbDockerfilesBinnacle},
        visualization depends on=rawy \as \myy,
        nodes near coords={\pgfmathprintnumber[fixed, precision=1]\pgfplotspointmeta\%},
        every node near coord/.style={
            color = gray,
            %   rotate=90,
            %   anchor=west,
            %   yshift=0.2cm
          },
        ymajorgrids = true,
        scaled ticks=false, tick label style={/pgf/number format/fixed},
        xtick style={draw=none},
        xticklabels = \empty,
        extra x ticks = \empty,
        extra x tick labels = \empty,
        legend style={draw=none}
      ]
      \addplot+[mark=none, rot_8a, very thick] coordinates { (0, 77576) (1, 36976) (2, 19886) (3, 11598) (4, 28335) (5, 3053) (6, 886) (7, 142)};
      \addlegendentry{Binnacle Dataset}
      %       \addplot+[mark=none, white, very thick] coordinates { };
    \end{axis}
  \end{tikzpicture}\vspace{-1em}
\begin{tikzpicture}
    \begin{axis}[
        ybar,
        xmin = -0.5,
        xmax = 7.5,
        ymin = 0,
        %       ymax = 35,
        bar width = 6.5mm,
        axis x line* = bottom,
        axis y line* = left,
        % y axis line style= { draw opacity=0 },
        % ytick=\empty,
        ylabel= \# Dockerfiles,
        xlabel= \# smell per Dockerfile,
        width= 0.48\textwidth,
        height = 0.22\textwidth,
        point meta={y*100/\nbParfumDockerfiles},
        visualization depends on=rawy \as \myy,
        nodes near coords={\pgfmathprintnumber[fixed, precision=1]\pgfplotspointmeta\%},
        every node near coord/.style={
            color = gray,
            %   rotate=90,
            %   anchor=west,
            %   yshift=0.2cm
          },
        scaled ticks=false, tick label style={/pgf/number format/fixed},
        ymajorgrids = true,
        xticklabels = \empty,
        extra x ticks = {0,1,2,3,4,5,6,7},
        extra x tick labels = {0,1, 2, 3, 4-10, 10-20, 20-50, > 50},
        legend style={draw=none}
      ]
      \addplot+[mark=none, blau_1a, very thick] coordinates { (0, 83461) (1, 35417) (2, 26456) (3, 16931) (4, 26192) (5, 4015) (6, 1179) (7, 297)};
      \addlegendentry{\tool Dataset}
      %       \addplot+[mark=none, white, very thick] coordinates { };
    \end{axis}
  \end{tikzpicture}
  \caption{The distribution of the number of smells detected by \tool per Dockerfile on the two datasets.}
  \label{fig:distribution_smell_binnacle_dataset}
\end{figure}

% \begin{figure}[t] 
%   \centering
%   \begin{tikzpicture} 
%     \begin{axis}[
%       ybar,
%       xmin = -0.5,
%       xmax = 7.5,
%       ymin = 0,
% %       ymax = 35,
%             bar width = 6.5mm,
%       axis x line* = bottom,
%       axis y line* = left,
%             % y axis line style= { draw opacity=0 },
%             % ytick=\empty,
%       ylabel= \# Dockerfiles,
%       xlabel= \# violations,
%       width= 0.48\textwidth,
%       height = 0.32\textwidth,
%       point meta={y*100/\nbDockerfiles},
%       visualization depends on=rawy \as \myy,
%             nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%},
%       every node near coord/.style={
%           color = gray,
%        %   rotate=90,
%        %   anchor=west,
%        %   yshift=0.2cm
%       },
%       ymajorgrids = true,
%       xticklabels = \empty,
%             extra x ticks = {0,1,2,3,4,5,6,7},
%       extra x tick labels = {0,1, 2, 3, 4-10, 10-20, 20-50, > 50},
%       ]
%       \addplot+[mark=none, blau_1a, very thick] coordinates {(0, 180177) (1, 5638) (2, 4865) (3, 1322) (4, 1620) (5, 219) (6, 31) (7, 1)};
% %       \addplot+[mark=none, white, very thick] coordinates { };
%     \end{axis}
%   \end{tikzpicture}
%   \caption{Distribution of the number of violations per Dockerfile inside the new dataset of Dockerfiles after repair}
%   \label{fig:nb_restarted_project}
% \end{figure}

==> macros.tex <==
\def\tool{\texttt{Parfum}\xspace}
\def\astTool{Dinghy\xspace}

\makeatletter
\@ifclasswith{acmart}{anonymous}{%
\def\urlDemo{https://anonymous.4open.science/w/docker-parfum/}%
\def\urlTool{https://anonymous.4open.science/r/docker-parfum/}%
\def\urlExpe{https://anonymous.4open.science/r/docker-parfum-experiment-BC2F/}%
\def\urlASTTool{https://anonymous.4open.science/r/Dinghy/}%
}{%
\def\urlDemo{https://durieux.me/docker-parfum}%
\def\urlTool{https://github.com/tdurieux/docker-parfum}%
\def\urlExpe{https://github.com/tdurieux/docker-parfum-experiment}%
\def\urlASTTool{https://github.com/tdurieux/Dinghy}%
}
\makeatother


\def\nbRule{14}
\def\nbSupportedCmd{88}

%RQ1
\def\totalDockerDiff{17715}
\def\totalSmellyDockerFileByToolInBinnacle{75454}
\def\totalSmellyDockerFileByBinnacleInBinnacle{72313}
\def\totalDiff{49337}
\def\nbViolationsByTool{235948}
\def\nbViolationsByBinnacle{197271}

\def\nbTotalDockerfiles{338211}
\def\nbBinnacleDockerfiles{178463}
\def\nbParfumDockerfiles{159748}
\def\nbTotalDockerfilesWithSmell{164597}
\def\nbBinnacleDockerfilesWithSmell{75454}
\def\nbParfumDockerfilesWithSmell{89143}

\def\nbTotalRepairedDockerfiles{338211}
\def\nbBinnacleRepairedDockerfiles{178463}
\def\nbParfumRepairedDockerfiles{159748}
\def\nbTotalRepairedDockerfilesWithSmell{492}
\def\nbBinnacleRepairedDockerfilesWithSmell{233}
\def\nbParfumRepairedDockerfilesWithSmell{259}


% RQ2
\def\totalRepairTime{1d 10h 16m 40s 952ms\xspace}
\def\avgRepairTime{365ms\xspace}
\def\nbSmell{514793}
\def\nbSmellAfterRepair{783}
\def\nbSmellyDockerAfterRepair{492}
\FPeval{nbRepairedSmell}{round(\nbSmell - \nbSmellAfterRepair,0)}



\def\countBuildError{369}
\def\countBuildableDockerfile{5196}
\def\countBuildedDockerfile{11313}
\FPeval{countBuildableDockerfileAfterRepair}{round(\countBuildableDockerfile - \countBuildError,0)}
\def\executionTime{\np[days]{41.5}}
\def\avgExecutionTime{8m 37s\xspace}


% RQ3
\def\nbDockerHub{1511}

\def\nbSmellInBuildable{21165}
\def\nbSmellInRepaired{5020}
\def\nbRepairedSmellInBuildable{16145}
\def\nbSmellInDockerHub{2075}
\def\nbRepairedSmellInDockerHub{889}

\def\totalSize{\np[TB]{5.56}}
\def\totalSpaceSaved{\np[GB]{277.03}}
\def\avgSpaceSaved{\np[MB]{48.06}}
\def\medSpaceSaved{\np[MB]{1.9}}
\def\maxSpaceSaved{\np[GB]{6.66}}

\def\totalPull{3446722231}
\def\totalPullWeek{11784785}
\def\totalSaved{\np[GB]{277.03}}
\def\totalSavedWeek{\np[TB]{40.45}}

%RQ4
\def\nbPRs{34}
\def\nbAcceptedPR{26}
\def\nbRefusedPR{2}
\def\nbMergedRepairedSmell{78}
\def\totalSpacePR{\np[GB]{21.08}}
\def\totalSpaceMerged{\np[GB]{3.46}}
\def\totalSpaceSavedPerWeek{\np[TB]{2.05}}
\def\mergedDownloadTimeWeek{45617}


\FPeval{nbPendingPR}{round(\nbPRs - \nbAcceptedPR - \nbRefusedPR,0)}


% Dataset
\def\nbDockerfilesBinnacle{178452}
\def\nbDockerfilesByTool{178463}
\def\nbDockerfilesGroundTruth{384}
\def\nbDockerfilesGroundTruthWithSmell{152}

==> tables/old_smell_table.tex <==
\begin{table}[ht]
    \centering
    \caption{Supported Docker smells and its origin.}\label{tab:rules}
    \begin{tabularx}{\linewidth}{@{}r X l@{}}
\toprule
ID & Smell Description & Origin\\
\midrule
1   & \code{curl} follows HTTP redirections. & Binnacle \\
2   & Use \code{curl -f} to prevent failing HTTP requests. \\
3   & All \code{apt-get install} should group into one. \\
4   & Clean cache after \code{npm install}. \\
5   & Force to clean cache after \code{npm install}. \\
6   & Clean cache after \code{yarn install}. \\
7   & Remove temporary folders. \\
8   & Use HTTPS in \code{curl}. \\
9   & Use HTTPS in \code{wget}. \\
10  & Clean cache after \code{pip install}. \\
11  & Remove /usr/src/* after usage. \\
12  & Use \code{--build} flag in \code{./configure}. \\
13  & Clean cache after \code{gem update --system}. \\
14  & \code{sha256sum} uses one space as a separator. \\
15  & Add \code{--no-document} flag to the .gemrc config file. \\
16  & Remove .asc file after usage. \\
17  & Use \code{-y} flag in \code{yum install}. \\
18  & Clean cache after \code{yum install}. \\
19  & Remove tar files after decompression. \\
20  & Use \code{--batch} flag in \code{gpg} in Docker. \\
21  & Use ha.pool.\_ instead of pool.\_ in \code{gpg}. \\
22  & Use \code{-y} flag in \code{apt-get install} \\
23  & Use \code{--no-install-recommends} flag in \code{apt-get install}. \\
24  & Run \code{apt-get update} and \code{install} in a single layer. \\
25  & Remove \code{/var/lib/apt/lists/*} after \code{apt-get install}. \\
26  & Use \code{--no-cache} flag with \code{apk add}. \\
27  & Do not use the root user in Dockerfiles. \\
28  & Do not use \code{sudo}. \\
29  & Use \code[dockerfile]{COPY} instead of \code[dockerfile]{ADD} for files and folders. & Hadolint \\
30  & Use apt-get and apt-cache instead of \code{apt}. & Hadolint\\
31  & Specify \code{--platform} in \code[dockerfile]{FROM} clause. & Hadolint\\
32  & Use the \code{--no-log-init} flag with \code{useradd}. & Hadolint \\
\bottomrule
\end{tabularx}
\end{table}

==> tables/violations_occurrence_binnacle.tex <==
\begin{table*}[t]
    \caption{Number of smells and smelly Dockerfiles detected by Binnacle and \tool on the Binnacle dataset. The total diff numbers represent the sum of absolute differences.}
    \label{tab:nbViolationBinnacle}
    \centering
    \begin{tabular}{@{}l r r r|r r r@{}}
    \toprule
\multirow{2}{*}{Docker Smell} &  \multicolumn{3}{c|}{\# Docker Smell}  & \multicolumn{3}{c}{\# Dockerfile with Smell} \\
&  Binnacle \cite{10.1145/3377811.3380406} &  \tool  & Diff &  Binnacle \cite{10.1145/3377811.3380406} &  \tool & Diff\\\midrule
aptGetInstallUseNoRec & \percent{61836}{\nbViolationsByBinnacle} & \percent{78810}{\nbViolationsByTool} & \np{16974} & \percent{36770}{\totalSmellyDockerFileByToolInBinnacle} & \percent{40825}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{4055}\\
aptGetInstallThenRmAptLists & \percent{57079}{\nbViolationsByBinnacle} & \percent{73921}{\nbViolationsByTool} & \np{16842} & \percent{32349}{\totalSmellyDockerFileByToolInBinnacle} & \percent{36250}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{3901}\\
curlUseFlagF & \percent{50613}{\nbViolationsByBinnacle} & \percent{48423}{\nbViolationsByTool} & \np{-2190} & \percent{36968}{\totalSmellyDockerFileByToolInBinnacle} & \percent{36819}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-149}\\
pipUseNoCacheDir & \percent{29735}{\nbViolationsByBinnacle} & \percent{30133}{\nbViolationsByTool} & \np{398} & \percent{16568}{\totalSmellyDockerFileByToolInBinnacle} & \percent{16793}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{225}\\
gpgUseBatchFlag & \percent{29127}{\nbViolationsByBinnacle} & \percent{29110}{\nbViolationsByTool} & \np{-17} & \percent{10070}{\totalSmellyDockerFileByToolInBinnacle} & \percent{10069}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-1}\\
aptGetUpdatePrecedesInstall & \percent{27017}{\nbViolationsByBinnacle} & \percent{37942}{\nbViolationsByTool} & \np{10925} & \percent{13151}{\totalSmellyDockerFileByToolInBinnacle} & \percent{16517}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{3366}\\
npmCacheCleanAfterInstall & \percent{14149}{\nbViolationsByBinnacle} & \percent{14189}{\nbViolationsByTool} & \np{40} & \percent{10467}{\totalSmellyDockerFileByToolInBinnacle} & \percent{10486}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{19}\\
yumInstallRmVarCacheYum & \percent{12247}{\nbViolationsByBinnacle} & \percent{12277}{\nbViolationsByTool} & \np{30} & \percent{6102}{\totalSmellyDockerFileByToolInBinnacle} & \percent{6121}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{19}\\
curlUseHttpsUrl & \percent{12073}{\nbViolationsByBinnacle} & \percent{8401}{\nbViolationsByTool} & \np{-3672} & \percent{5166}{\totalSmellyDockerFileByToolInBinnacle} & \percent{5084}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-82}\\
apkAddUseNoCache & \percent{11430}{\nbViolationsByBinnacle} & \percent{6278}{\nbViolationsByTool} & \np{-5152} & \percent{8732}{\totalSmellyDockerFileByToolInBinnacle} & \percent{4860}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-3872}\\
configureShouldUseBuildFlag & \percent{9288}{\nbViolationsByBinnacle} & \percent{9505}{\nbViolationsByTool} & \np{217} & \percent{5422}{\totalSmellyDockerFileByToolInBinnacle} & \percent{5515}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{93}\\
wgetUseHttpsUrl & \percent{7461}{\nbViolationsByBinnacle} & \percent{7153}{\nbViolationsByTool} & \np{-308} & \percent{4934}{\totalSmellyDockerFileByToolInBinnacle} & \percent{4730}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-204}\\
tarSomethingRmTheSomething & \percent{5096}{\nbViolationsByBinnacle} & \percent{10841}{\nbViolationsByTool} & \np{5745} & \percent{3465}{\totalSmellyDockerFileByToolInBinnacle} & \percent{7785}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{4320}\\
gpgUseHaPools & \percent{3338}{\nbViolationsByBinnacle} & \percent{3332}{\nbViolationsByTool} & \np{-6} & \percent{1155}{\totalSmellyDockerFileByToolInBinnacle} & \percent{1154}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-1}\\
mkdirUsrSrcThenRemove & \percent{2666}{\nbViolationsByBinnacle} & \percent{2659}{\nbViolationsByTool} & \np{-7} & \percent{2458}{\totalSmellyDockerFileByToolInBinnacle} & \percent{2452}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-6}\\
aptGetInstallUseY & \percent{2251}{\nbViolationsByBinnacle} & \percent{5568}{\nbViolationsByTool} & \np{3317} & \percent{1741}{\totalSmellyDockerFileByToolInBinnacle} & \percent{3462}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{1721}\\
npmCacheCleanUseForce & \percent{1344}{\nbViolationsByBinnacle} & \percent{1354}{\nbViolationsByTool} & \np{10} & \percent{1323}{\totalSmellyDockerFileByToolInBinnacle} & \percent{1333}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{10}\\
rmRecursiveAfterMktempD & \percent{1187}{\nbViolationsByBinnacle} & \percent{397}{\nbViolationsByTool} & \np{-790} & \percent{296}{\totalSmellyDockerFileByToolInBinnacle} & \percent{292}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-4}\\
sha256sumEchoOneSpaces & \percent{881}{\nbViolationsByBinnacle} & \percent{2243}{\nbViolationsByTool} & \np{1362} & \percent{409}{\totalSmellyDockerFileByToolInBinnacle} & \percent{1916}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{1507}\\
gemUpdateSystemRmRootGem & \percent{249}{\nbViolationsByBinnacle} & \percent{246}{\nbViolationsByTool} & \np{-3} & \percent{231}{\totalSmellyDockerFileByToolInBinnacle} & \percent{229}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-2}\\
gemUpdateNoDocument & \percent{161}{\nbViolationsByBinnacle} & \percent{158}{\nbViolationsByTool} & \np{-3} & \percent{145}{\totalSmellyDockerFileByToolInBinnacle} & \percent{143}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-2}\\
gpgVerifyAscRmAsc & \percent{92}{\nbViolationsByBinnacle} & \percent{85}{\nbViolationsByTool} & \np{-7} & \percent{90}{\totalSmellyDockerFileByToolInBinnacle} & \percent{83}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{-7}\\
yumInstallForceYes & \percent{18}{\nbViolationsByBinnacle} & \percent{18}{\nbViolationsByTool} & \np{0} & \percent{15}{\totalSmellyDockerFileByToolInBinnacle} & \percent{15}{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{0}\\
\midrule
Total & \np{\nbViolationsByBinnacle} & \np{\nbViolationsByTool} & \np{\totalDiff} & \np{\totalSmellyDockerFileByBinnacleInBinnacle} & \np{\totalSmellyDockerFileByToolInBinnacle} & \np{\totalDockerDiff} \\
\bottomrule
    \end{tabular}

\end{table*}
